Distance Assisted Recursive Testing

In many applications, a large number of features are collected with the goal to identify a few important ones. Sometimes, these features lie in a metric space with a known distance matrix, which partially reflects their co-importance pattern. Proper use of the distance matrix will boost the power of identifying important features. Hence, we develop a new multiple testing framework named the Distance Assisted Recursive Testing (DART). DART has two stages. In stage 1, we transform the distance matrix into an aggregation tree, where each node represents a set of features. In stage 2, based on the aggregation tree, we set up dynamic node hypotheses and perform multiple testing on the tree. All rejections are mapped back to the features. Under mild assumptions, the false discovery proportion of DART converges to the desired level in high probability converging to one. We illustrate by theory and simulations that DART has superior performance under various models compared to the existing methods. We applied DART to a clinical trial in the allogeneic stem cell transplantation study to identify the gut microbiota whose abundance will be impacted by the after-transplant care.

==> sections/acknowledgement.tex <==
\section*{Acknowledgment}

The microbiome samples were collected and sequenced at Memorial Sloan
Kettering Cancer Center (MSKCC) and pre-processed at Duke Cancer
Institute (DCI) Bioinformatics Shared Resource (BSR).  We thank Tsoni
Peled and Marcel van den Brink from MSKCC for sample collection and
sequencing. We thank Kouros Owzar and Alexander Sibley from DCI-BSR
for data pre-processing, helpful discussions, and support.  Xuechan Li
and Jichun Xie's research is supported by Jichun Xie's startup fund
from Duke University. Anthony Sung's research is supported by NIH Award 1-R01-HL151365.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../manu"
%%% End:


==> sections/manu.tex <==

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:

